Participation in the age of foundation models

Growing interest and investment in the capabilities of foundation models has positioned such systems to impact a wide array of public services. Alongside these opportunities is the risk that these systems reify existing power imbalances and cause disproportionate harm to marginalized communities. Participatory approaches hold promise to instead lend agency and decision-making power to marginalized stakeholders. But existing approaches in participatory AI/ML are typically deeply grounded in context - how do we apply these approaches to foundation models, which are, by design, disconnected from context? Our paper interrogates this question. First, we examine existing attempts at incorporating participation into foundation models. We highlight the tension between participation and scale, demonstrating that it is intractable for impacted communities to meaningfully shape a foundation model that is intended to be universally applicable. In response, we develop a blueprint for participatory foundation models that identifies more local, application-oriented opportunities for meaningful participation. In addition to the "foundation" layer, our framework proposes the "subfloor'' layer, in which stakeholders develop shared technical infrastructure, norms and governance for a grounded domain, and the "surface'' layer, in which affected communities shape the use of a foundation model for a specific downstream task. The intermediate "subfloor'' layer scopes the range of potential harms to consider, and affords communities more concrete avenues for deliberation and intervention. At the same time, it avoids duplicative effort by scaling input across relevant use cases. Through three case studies in clinical care, financial services, and journalism, we illustrate how this multi-layer model can create more meaningful opportunities for participation than solely intervening at the foundation layer.

==> sections/OLD/case-study_finance.tex <==

\subsection{Case Study 2: Financial services}
In our second case study, we examine a case of a financial services provider who is seeking to explore the use of generative AI for fraud detection. Every payment network assigns risk scores to each transaction based on data available at the point of sale such as the amount, the frequency, and the pattern of transactions. This risk score is reported by the payment network to the issuing bank, which can decide to process or decline the transaction. Large banks like Chase and Citigroup can accept more risk and set their risk threshold higher; smaller issuers like credit unions may not be able to take on as much risk and set lower thresholds.
% When a customer makes a purchase at a merchant, that shop has an ``acquiring bank'' that submits the transaction to the customer's ``issuing bank'' over a payment network like Mastercard or Visa, which pulls funds from the customer's account at the issuing bank (REF). 
In the wake of GPT3.5, which was released to the public in late 2022, major financial firms began to explore the use of large language models for improving performance of fraud detection scoring.

\textbf{The problem.} Financial services providers recognize the enormous fairness and equity risks of fraud detection algorithms and risk scoring. Credit card issuing banks and payment networks are concerned with protecting their reputations; assessment procedures are designed to avoid declining transactions in a frivolous or inequitable way. While financial services providers are interested in the potential for large language models to improve the accuracy of fraud detection, deep learning techniques' increased stochasticity and complexity also increases the risk of violating the law or and other fairness commitments. 

In the United States, federal authorities like the Federal Trade Commission and laws like the Equal Credit Opportunity Act (ECOA) hold credit card companies accountable for credit discrimination. These laws, as well those for consumer protection and preventing financial system risk, establish a complex set of regulatory requirements that financial services firms must operate within. 

This legal context and the intellectual property protections in place at these firms make it more challenging for banks and payment providers to evaluate the risk and promise of large language models for fraud detection. Evaluations are conducted strictly behind closed doors to protect firm competitiveness. Open information sharing between rival firms would raise antitrust concerns; as a result, the risks that LLMs could pose to communities via false positives in fraud detection and inequitable credit service provision are underexamined---\textit{particularly by the communities who would be most affected and the organizations that represent them.}

\textbf{The opportunity.} In this case, our framework would guide multiple financial services providers---who must both adhere to federal law and ethical requirements for fairness and equity---to seek opportunities to make the LLMs being used in their products and services more porous to public input. We propose the subfloor layer as a series of working groups and deliberative bodies organized around an institutional body already common to financial services providers: for instance, the Payment Card Industry (PCI) Security Standards Council is a standards-making body that consistently convenes and issues guidance to financial services firms on information security and privacy protections for every aspect of the card and network, from the plastic material, to the magnetic strip, chip, information encoding, network protocols, and more. 

Guidance and resources issued by the PCI Security Standards Council are both technical and non-technical; the body helps to establish best practices across the payment system architecture. By hosting global events and working groups that advise all companies at once, PCI is able to avoid the antitrust concerns that would arise in the event that financial services firms elected to partner or collaborate with other firms directly. Its remit is also inclusive of best practices for new tools and technologies like generative AI.

Importantly, a version of the subfloor layer that would iteratively change the design of an LLM is heavily constrained by the financial services context. Fraud detection algorithms used in the network are embedded in complex relationships between the payment network, acquiring banks, issuing banks, merchants, and customers. Substantive changes to the model itself would require the re-negotiation of an equally vast number of vendor agreements between the payment network and banks.

A subfloor layer as hosted by a neutral third party resource like PCI is an example of the value instead of \textit{non-technical contributions} to identifying LLM risks and harms. For example, PCI already exists to facilitate knowledge transfer between industry players and to diffuse findings from special collaborations, working groups, and programming. We propose that the existing set of special interest groups hosted at PCI be broadened to include civil society and advocacy organizations, financial wellness community groups, and others who can inform industry understanding of the risks of LLMs as they relate to high-stakes uses and vulnerable communities.

Cohering subfloor interventions into known harms, system vulnerabilities, and other issue areas is a more flexible output of participation at the subfloor layer. The intended audience for these findings would be in-house counsel, privacy and risk management personnel, and regulatory teams, who can in turn diffuse these known harms into guidance and ready-at-hand advice to product teams who create or adapt LLMs for financial services uses.

\textbf{Participatory methods.} In this case study, financial services firms like banks and payment providers were unable to make the LLMs they are evaluating porous to public input, in spite of the high stakes and enormous risks of inequitable outcomes. Here, the subfloor layer is a primarily organizational infrastructure that convenes key stakeholders for working groups that identify community concerns and potential harms. This set of consultative relationships allows financial firms to take on additional external input in spite of a highly closed and rigid overall environment. This wider set of expertise and interested publics enrolled in identifying risks is able to inform and guide products and services while being compatible with established legal and organizational constraints. 


==> sections/OLD/old-case-study-healthcare.tex <==
\subsection{Case study 1: Clinical care}

Our first case study examines how healthcare providers might use generative AI during the clinical encounter between a healthcare provider and their patient.
Decades of digitization have added enormous documentation burden to the everyday work of medical doctors, nurses, and other clinical practitioners, whose labor is now mediated in large part by the electronic health record (EHR) \cite{gawande2018doctors}.
A visit to the doctor's office now consists of a patient sitting on an exam table while a doctor types away on a screen or a tablet, in an appointment slot that can be just 15 minutes.
Clinicians now work email jobs, too: between exam-room shifts, they are inundated with patient messages, often with an expectation to answer thoughtfully within 1-3 business days. 

Towards freeing clinicians' time from documentation and email towards patient interaction, researchers and practitioners have long explored tools for machine assistance in clinical care.
Chatbots backed by decision trees are used to route patients to the right provider.
The basic clinical task of taking faithful, informative, and structured clinical notes has been augmented with tools like templates injected into patient records, or dictation apps backed by automatic speech recognition (ASR).
For more advanced tasks like identifying the right diagnosis or ordering the right battery of tests, EHRs have introduced embedded checklists and recommendation systems that aim to minimize medical errors while improving doctors' efficiency.
The need in this area has been so great that entire human workforces have been invented to ease clinicians' administrative burden, including roles for medical scribes and medical billing coders.

Efforts to improve efficiency in clinical care were turbocharged by the mainstream release of OpenAI's ChatGPT. In 2023, EHR providers began announcing generative AI integrations and live pilot studies with healthcare systems all over the U.S.
Oracle released a Clinical Digital Assistant product within its EHR that could automate note-taking as well as ``\textit{propose context-aware next actions, such as ordering medication or scheduling labs and follow-up appointments}'' \cite{oracle2023generative}.
Epic partnered with Microsoft to launch generative AI-powered message handling in a series of pilots with health systems at UNC, UC San Diego, Stanford and the University of Wisconsin \cite{epic2023generative}.
LLM-powered tools have additionally been proposed to assist in the routine labor of medical billing, in clinicians' assessments of clinical evidence, and in understanding biomedical literature.

\paragraph{The problem} LLM-powered tools promise to ease clinicians' burdens, and therefore improve the quality of care experienced by all patients.
Fulfilling this premise requires the builders of LLMs to devote careful attention to fairness and equity---for both the \textit{providers} whose decision-making would be augmented by these tools, and the \textit{patients} who would bear the weight of what can be life-altering decisions made by these combined human-AI systems.

First, the builders of LLM-powered tools must ensure their products improve clinicians' workplace performance and well-being, rather than imposing greater cognitive burden.
There is the issue of trust: whether providers can believe an LLM-powered tool's recommendations.
LLMs are known to hallucinate, and providers could find themselves ignoring their suggestions to avoid the threat of malpractice, or devoting additional time to verifying their suggestions. 
% \enote{to my knowledge, this is actually not yet addressed in case law, although it is for lawyers; we could strike the malpractice note if we don't need it} 
At a higher level, clinicians are a frontline workforce consisting of teams with strict hierarchies, and technologies that shape their collaborative work practices can improve efficiencies for some team members at the expense of others.
For example, an attending physician might use an LLM-powered dictation tool for note-taking throughout their shift, but still require a resident or scribe to sift through the day's raw transcripts to verify the LLM's correctness.

On the patients' side, LLM builders must ensure these tools do not exacerbate long-documented inequities in the healthcare system, e.g., biases in risk scoring algorithms that result in disparate treatment and outcomes for people experiencing marginalization \cite{eneanya2019reconsidering}.
% Scholars of health equity have established how discrimination manifests throughout healthcare in poorer treatment and outcomes for marginalized people.
Without the tools to audit and assure LLM outputs can be reasonably equitable, we risk enabling clinicians to overrely on biased technology and issue the wrong treatments to patients from marginalized communities.
Lastly, at a systemic level, LLM-powered clinical services threaten to widen disparities in access to quality care.
A healthcare system could, for example, provide an LLM-powered medical advice chatbot in lieu of hiring more providers. 
While wealthier patients will always be able to find and access high-quality, specialized, and in-person care, we risk normalizing stopgap measures like chatbots as the standard of care for lower-income patients.

\paragraph{The opportunity} Our blueprint would guide the builder of a clinical care LLM to \textit{incorporate feedback from diverse stakeholders, with potentially competing interests}, by composing between the subfloor and application levels. 
Clinical care is already organized around standards of care and licensure at multiple levels of organization, e.g., national and state-level guidance.
Given a task (e.g., ``an LLM-based chatbot to inform a patient of post-surgical care after cardiovascular surgery''), an LLM tool developer might start by establishing an \textit{application layer} primarily concerned with context-specific logic, e.g., resources and procedures specific to a given hospital. 
This application layer could build from a \textit{subfloor layer} organized and maintained by a national governing body with expertise in the domain of that task, e.g., the subfloor for LLMs making recommendations in cardiology workflows could be managed by the American College of Cardiology. 
The subfloor model would unite expertise from different contexts to improve the LLM's performance on that task, while leaving room for the application-level model to incorporate local context.

Importantly, our framework gives room for  stakeholders at each level to weigh in on the LLM tool's fairness and equity, in terms of both its task-specific performance \textit{and} its effects on human workflows.
At the application layer, the LLM builder might convene organizational stakeholders including the administrative and clinical leadership of that hospital, as well as representatives from its staff and local patient population.
These stakeholders could participate in shaping the expected behavior for the tool \textit{and} report the ensuing errors or harms. Importantly, this convening could be where local stakeholders come to consensus over disputes between stakeholder groups: e.g., a hospital's administrators and nursing leadership can discuss how to organize a shift schedule for nurses to supervise the chatbot for post-surgical care, and how to structure the underlying LLM accordingly.
At the subfloor layer, the subfloor convener---the stewards of expertise in a cross-domain task---could then enlist a broader range of stakeholders (e.g., health equity experts in addition to cardiologists), as well as experts in labor conditions for the providers implicated in the task (e.g., scholars of medical education for tasks that implicate medical residents, or representatives of healthcare workers' unions like 1199SEIU). 

\paragraph{Participatory methods} The nested subfloor-application structure proposed here enables composition between participation on two complementary axes. 
At the application level, participatory decision-making can provide a surface for stakeholders with competing interests to decide how an LLM-backed tool affects context-specific workflows (application-level).
At the subfloor level, correctness, fairness, and equitable treatment in task performance between contexts can be enforced---while also leaving room for forms of collective action.

% - APPLICATION: 
% -- Scope: LLM-based app built and maintained by your org's staff, using the subfloor's LLM. 
% -- Stakeholders: Your org's leadership. Representatives of your patients, physicians, nurses, etc.
% -- Meaningful participation: Fine-tuned on your org's ruleset and data. Harms reported to both application and subfloor maintainers.

% - SUBFLOOR: 
% -- Scope: LLM for clinical notes governed, maintained, and assured by a coalition of clinical care experts. 
% -- Stakeholders: Physicians, malpractice lawyers, expertise in health equity, maybe residency training/med-ed, health management
% -- Meaningful participation: setting norms and evaluation procedures




==> sections/OLD/old-current-state-of-play.tex <==
\section{Current state, limitations}
\hnote{Framing: foundation models vs LLMs?}
Foundation models afford a different set of opportunities for participation than existing case studies of ``participatory ML'' have thus far.  In a classic ML setup, the downstream task and users are typically known upfront.  Opportunities for participation and community-based co-determination might include affected communities shaping problem formulation, determining details of data collection and storage, contributing to data annotation, or providing insight into evaluations that best reflect real-world usage.  In the foundation model setup, on the other hand, downstream use cases are more disconnected from the model.  Indeed, a driving motivation behind the development of foundation models is the ability to perform well on any number of heretofore unseen applications. \hnote{explain why the tasks being a giant and unknown set makes it hard for participation} Moreover, to achieve this kind of large-scale generalizability, model and dataset sizes are orders of magnitude larger than previous iterations of ML.  It becomes much more challenging to building participatory mechanisms into data collection when models require billions of training examples, or to provide transparency into the behavior of a model with trillions of parameters.  In this section, we review the current state of ``participatory'' approaches in foundation model development.  We then analyze these attempts through the lens of the Parameters of Participation, a framework developed by Delgado et al. to describe the goals, scope, and methods of participatory initiatives in AI \& ML.  

\subsection{Methods}
To understand the state of participation in foundation model development, we looked to multiple sources.  Our aim was to find material broadly related to ``participation,'' regardless of its ultimate effectiveness at redistributing power (i.e., regardless of where it falls on the ladder of citizen participation).

Because much of foundation model development is focused in commercial companies, we compiled public-facing materials from prominent industry providers (OpenAI, Anthropic, Google, Meta, Hugging Face, Cohere).  To find relevant material, we navigated to each company's public research index. If possible, we used filters to narrow the set to those links related to AI, ML, and/or NLP.  We then manually filtered articles to those that described any form of using human input or feedback to shape some part of the model lifecycle.

To capture academic research, we also searched conference proceedings from top venues in AI, NLP, computer vision, AI ethics and fairness, and HCI (NeurIPS, ICML, ICLR, EMNLP, CVPR, FAccT, CHI). \hnote{should we search arxiv? this search in conf proceedings led to very few relevant results} We identified documentation/papers with the following filter: ``(\textit{participation} or \textit{participatory} or \textit{value alignment} or \textit{human feedback}) and (\textit{large language model} or \textit{foundation model}).''  Our filter includes terms such as ``value alignment'' and ``human feedback'' to capture the fact that much of the existing efforts are not explicitly referred to as ``participatory.'' Finally, we manually filtered the results to ensure that they described using human participation to shape some aspect of the model.  

We did not include: 1) work where the main human input is through using an existing dataset generated by humans (e.g., example); 2) work that applies existing human feedback methods as is (e.g., ) or builds tooling to support them (e.g., ); 3) work where the only human input is to generate evaluation metrics (e.g., ).  

This process led to \todo{NUM} public-facing industry documents, and \todo{NUM} academic conference papers (some of which are authored by industry actors).  To understand the state of play, we grouped these materials into categories that capture shared methodology (e.g., ``RLHF''), and described where along the ML lifecycle each category falls.  Then, to uncover limitations and gaps of the approaches, we characterized each along the axes defined by the Parameters of Participation ---  the goal (why is participation needed?), the scope (who is involved, and what is on the table?), and the form (what is the participatory process?).  

\subsection{Findings}
\subsubsection{The state of play}

To date, mechanisms for human input are concentrated at the model training stage, with some methods (e.g., red-teaming) also occurring during system monitoring.  Many of these efforts are framed through the goal of ``human value alignment.''  \hnote{Do we want to analyze the concept of "human value alignment" and how it leads to a conceptually different (and less meaningful, context-specific,etc) form of participation?} The primary categories of participation we find are: 

\todo{add a bunch of citations of examples to these categories}

\textbf{Data creation}. Though it is typically not the focus of most papers (and though we excluded papers where the sole human input was through an existing dataset), all the research we examined involves training or fine-tuning models on data that is generated by humans.  Most foundation models are trained on large web datasets, which include news and wikipedia articles, websites, books, articles, artwork, social media posts, or other content authored by people.  In most cases, the creators of this data are not attributed and are typically unaware of its usage.  Other human-generated datasets include those intended for fine-tuning or evaluating specific capabilities. 

\textbf{Reinforcement learning with human feedback (RLHF)}.  RLHF is framed as a way to align the outputs of LLMs with human values, such as ``helpfulness'' or ``harmlessness.'' It typically occurs during training, after an initial, pre-trained LLM has been created. While there are different variants of RLHF, the high-level common process involves having the model produce multiple outputs, and asking humans to choose between them.  These choices are then used to train a preference model, which goes on to be used as a reward function in a reinforcement learning process that shapes the LLM.  

\textbf{Rulesets}. A ruleset (sometimes referred to as a ``constitution'') comprises a set of values or principles that a foundation model should follow.  In practice, a ruleset is typically operationalized via an RLHF process.  However, rather than choose according to an implicit notion of goodness or a general value like ``helpfulness,'' human raters choose the better response with respect to a particular rule from the ruleset.  Rulesets have been derived in different ways. Some draw from existing law and policy, while others are based primarily on developer discretion.  In other cases, rulesets are informed via public input or focus groups.  

\textbf{Red-teaming}. Red-teaming, common in computer security, involves adversarially testing a model for errors or vulnerabilities.  Recently, companies involved in foundation model development have proposed recruiting external domain experts to inform red-teaming efforts.  There are also external, open-source red-teaming repositories.

\subsubsection{The participatory ceiling}
We further characterized the set of \todo{NUM} participatory efforts using the \textit{dimensions} and \textit{modes} of participation described in Delgado et al.'s Parameters of Participation.  The dimensions are framed as questions: 1) Why is participation needed? 2) What is on the table? 3) Who is involved? and 4) What form does participation take?  The answers to these questions are structured along a spectrum of four modes of participation, which span consultation (e.g., eliciting user preferences), inclusion (e.g., deliberation around specific design choices), collaboration (e.g., co-creation of design possibilities), and ownership (e.g., stakeholders shape the entire design process).  

We find that attempts at incorporating participation into foundation models are limited, in all dimensions, to the \textit{consult} and \textit{include} modes of participation (as opposed to the \textit{collaborate} and \textit{own} modes).  There is some variance amongst methods. For example, consider RLHF with crowdworkers with the aim producing coherent chatbot responses.  In this case, participation is needed to improve the user experience.  Very little is on the table --- participants are only able to provide some amount of training data, with no guarantees on if and how it will be used.  The participants themselves are crowd-workers recruited by the research team for discrete feedback.  And the form of participation is providing answers to an online survey.  In each of these dimensions, the approach falls in the \textit{consult} mode of participation --- participants input influences a narrow slice of the development lifecycle in a non-transparent way.  Other approaches vary along certain dimensions.  For example, in the case of rulesets derived through demographic focus groups, participants are recruited by the research team for expertise in a particular kind of lived experience, and the form of participation is deliberative focus groups.  Along these dimensions, the approach falls under the \textit{inclusion} mode of participation.  However, in other dimensions, it remains in the realm of the \textit{consult} mode.  For instance, not much is on the table --- ultimately, participant input will form a ruleset that may (or may not) be used by the research team to train a different version of the model.  Participants have little say regarding if this model is developed, what other data it is trained on, what it may be used for, if and how it should be deployed, et cetera.  

\includegraphics[width=\textwidth]{sections/figures/fig1.png}
\hnote{Add example citations to the diagram?}

Why are participatory approaches thus far limited to those that lend little power to stakeholders?  We argue that, due to the large-scale and context-agnostic nature of foundation models, there is an inherent \textit{participatory ceiling} on what is possible when directly intervening on the foundation model.

\paragraph{1. Meaningful participation is inherently context-specific.}
-- Values, norms, culture differs across contexts 
-- Affected populations differ across contexts 
-- Context makes thinking about values and harms concrete, rather than abstract
-- Empathy gap 

\paragraph{2. Participation requires affected individuals to take on additional responsibility that can be burdensome or even unwanted} \todo{ET, based on citizen science and participatory data stewardship lit review}

\paragraph{3. Incentives are currently misaligned} 







==> sections/old235and33.tex <==


\subsubsection{Summary}

Looking across the approaches described above, we find the vast majority exhibit consistent limitations in how participatory foundation models can be. Analyzed through the lens of \citet{delgado2023participatory}'s Parameters:


\paragraph{Stakes} Foremost, the stakes of participation (i.e., ``what is on the table?'') are limited to the \textit{consultation} mode. 
%typically focused on model adjustments and controlled by the development team. 
% Significant effort is placed into generating rulesets in a more participatory way---
% However, optimizing the model is just one part of a much wider life cycle. 
In most approaches, participatory engagement is limited to generating rulesets, guidelines, or harms that shape model adjustments, rather than higher-level decisions, e.g., decisions about data sources or quality, or motivating factors for if and why a system should be built.  In some cases, methods do aim to expand the stakes, engaging participants in questions related to deployment, data quality, or appropriate use cases.  However, participants lack a degree of control (and the foundation model ecosystem lacks sufficient accountability mechanisms) that is crucial for these guidelines or findings to actually impact broader changes during development or deployment.  

% \enote{I might suggest reworking this to say, there's a bunch of effort on generating rulesets, but few accountability mechanisms}

\paragraph{Scope} When it comes to the \textit{scope} of people involved, there is some variance, including crowd-workers, domain experts, the general public, or identity-based groups.  While some of these approaches improve on upon others by soliciting diverse expertise (e.g., focus groups centered around marginalized identities) rather than primarily extracting labor (e.g., RLHF with crowd-workers), they remain capped at the \textit{inclusion} mode of participation.  In almost all examples we found, the expertise required and participants involved are determined by the development team, or via crowdsourcing, rather than stakeholders being designated by external affected communities.  

\paragraph{Form} Across examples, the \textit{form} of participation is designated by the development team, and spans from one-time online surveys (\textit{consult}) to group discussions over a short time frame (\textit{include}).  Participants typically do not have the opportunity to continue to have a voice in the process (\textit{collaborate}), or to have a say in how the participatory approach itself is structured (\textit{own}).  

\paragraph{Goal} All of these factors led us to conclude that across current examples, the \textit{goals} of participation at best aim to align the model with stakeholder preferences/values (\textit{include}), rather than to deliberate about system capabilities (\textit{collaborate}) or to ``shape the system's scope and purpose'' (\textit{own}).  

\subsection{The participatory ceiling}

\todo{expand with ubuntu example}
Why are participatory approaches thus far limited to those that lend little power to stakeholders?  We argue that, due to the large-scale and context-agnostic nature of foundation models, there is an inherent \textit{participatory ceiling} on what is possible when directly intervening on the foundation model.  

\paragraph{Incentives and organizational structures are currently misaligned}
We also note organizational constraints at the foundation layer that constrain the use of public participation. Indeed, the same challenges are present in any  organization developing or deploying AI. To date, large technology development firms like Microsoft and Intel have sought to establish that they are not liable for the downstream uses of their products. Where a firm does not accept ultimate liability for harm, it has less incentive to collaborate with impacted communities to identify and prevent it. Moreover, most large organizations are risk-averse: partnerships with advocacy groups (or public ethics advisory boards) create openings for the company to be publicly criticized, or exposed to federal regulation and enforcement. If meaningful participation requires the distribution of some decision-making power, this shift is not easily available to firms, which are primarily constituted to protect shareholder interests. There are also practical challenges: overcoming intellectual property barriers and integrating user feedback into data science engineering are both known challenges across responsible AI work. We note that these constraints deepen a tendency to atomize participation into discrete input from individual users, rather than sustain participation via long-term inter-organizational partnerships.
%may be more realistic in non-profit, university, and governmental initiatives 


\paragraph{Meaningful participation necessitates context-specificity}
Unlike traditional AI/ML models where datasets, modeling, and evaluation are centered around a specific task, foundation models are intended to be generally applicable across domains, geographies, and other contexts.  Therefore, most of the participatory efforts we surveyed aimed to construct general, universally-applicable rules or guidelines. 

The participatory tradition, however, has historically been grounded in \textit{context-specificity}. Prioritizing context in fields such as Participatory Action Research (PAR) stems from the acknowledgement that local stakeholders (i.e., people embedded in the day-to-day of a particular context) hold complex and valuable expertise about the needs, dynamics, and intricacies of their environment \cite{greenwood2006introduction}.  It also acknowledges that local knowledge systems are differentiated and non-interchangeable; values or norms in one context may not neatly transfer to another.  The same holds for understanding how harm manifests --- as described in intersectional feminist theory, the reality of marginalization is highly varied \cite{collective1977combahee, collins2019intersectionality, crenshaw2013mapping,d2023data}.  Considering context lends concreteness to \textit{what} harm actually looks like in a grounded domain and \textit{who} may be disproportionately affected.  Finally, from a cognitive psychology perspective, grounding deliberation in familiar and realistic situations is important for eliciting accurate perceptions. As work in human-computer interaction (HCI) has shown empirically, the ways people react to and think about AI systems changes depending on whether they are engaged in an abstracted proxy task versus a more realistic, application-grounded task \cite{buccinca2020proxy,doshi2018considerations}. 

%A focus on context and local, tacit knowledge can reveal, for example, how 

When participatory efforts aim to produce universal outputs, they no longer prioritize local knowledge.  Instead, they ask participants to reason about hypothetical, distant, or abstract scenarios.  This is challenging cognitively: consider a high-school teacher reasoning about whether ``respect'' or ``honesty'' is a more important value for an LLM to adhere to, versus considering the concrete tradeoffs and risks of an LLM-based tutoring tool integrated into their classroom.  It may also lead to outputs that do not reflect actual downstream needs.  

More broadly, the methods we surveyed tend to reflect an approach to participation that views model builders as the stewards of expertise, responsible for eliciting preferences from people and shaping the model \textit{for} them. An approach that instead acknowledges downstream stakeholders as experts on local knowledge systems---who are much better suited to understand how a system might succeed or fail in their context---suggests lending participants much higher levels of control, conceptualizing the system's scope and purpose \textit{with} them.  


\paragraph{Participation can be burdensome} 
Lastly, efforts towards participatory foundation models must contend with a practical reality: asking affected communities to participate in technology design may be so laborious that it becomes an unwanted burden.
Whether at the atomized level of an individual vote or in a deliberative process of collective consensus \cite{frischmann2014governing}, any participatory design process demands time, energy, and effort from participants, in both material and affective terms \cite{dourish2020being}, and demanding this labor from people already facing marginalization may exacerbate the harms they face \cite{dombrowski2016social}.
Foundation models are also a new technology subject to tremendous hype in the popular press under the banner of general artificial intelligence, and their governance thus requires a willingness to speculate on future risks and possibilities.
While such speculation can lead to greater technological awareness and literacy, 
\citet{harrington2019deconstructing} argue that asking marginalized communities to the ``\textit{blue-sky ideation}'' of design speculation risks ultimately frustrating underserved individuals, who contend with real and grievous harms in everyday life.


\todo{Notably, one example out of those surveyed seemed to indicate a more participatory mode of engagement: UbuntuAI, which does this and has these nice properties. How structures like UbuntuAI can be replicated more broadly is the subject of the next section.}


==> sections/tab-foundation-problems.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table}[t]
\centering
\small
\renewcommand{\arraystretch}{1.2}

% \resizebox{\columnwidth}{!}
{%
\begin{tabular}{m{2.7cm} m{5cm} @{\hskip 1cm} >{\arraybackslash}m{6cm}}
\toprule
 & \multicolumn{2}{c}{{\ul \textbf{Is Participation Tractable?}}} \\
\textbf{Phase of ML lifecycle} & \textbf{Task-Specific Paradigm} & \textbf{Foundation Model Paradigm} \\ \midrule
Problem Formulation & Yes. Context-specificity means communities can deliberate over task-appropriateness. 
% (In a task-specific paradigm, grassroots control of an ML pipeline is possible) 
& No. A model is trained to represent the knowledge in its training data, and then used for an unbound range of downstream tasks. 
% (Grassroots control not possible bc by definition need central powerful authority)
% Deliberation is possible at fine-tuning, but models may inherit biases from the foundation layer that have bearing on task-appropriateness.
\\ \midrule
Dataset Curation & Yes. Participatory ML has explored ways to encourage participation in collection, curation, and annotation. & Unclear. Foundation models embed Internet-scale datasets that may be too large and general-purpose for existing methods of inspection or audit. 
% And fine-tuned models may be annotated or curated in a participatory fashion, but would still inherit all the issues of their foundation dataset.  (Section 3) 
\\ \midrule
Model Development & Yes. Participation might shape training iterations, optimization constraints, or interpretability mechanisms.   & Unclear. Work has proposed adjusting models with RLHF (\ref{sec:rlhf}) or rulesets (\ref{sec:rulesets}), but do these work for an unknown horizon of possible future uses and reliance on a universal model provider?   \\ 
\midrule
Evaluation and Deployment & Yes. Participatory ML has explored methods such as curated benchmarks, public auditing \& accountability mechanisms, and sustained partnerships in deployment.  & Unclear. Work has proposed general guidelines (\ref{sec:rulesets}), red-teaming (\ref{sec:redteaming}) or crowdsourced benchmarks (\ref{sec:domainharms}), but do these work for an unknown horizon of possible future uses and reliance on a universal model provider? \\ 
\bottomrule
\end{tabular}%
}
\caption{Comparison of participation tractability across model lifecycle stages for ML in the task-specific vs. foundation paradigm.}
\label{tab:comparison}
\vspace{-20pt}
\end{table}
